Assessing present and future risk of water damage using building attributes, meteorology and topography

Weather-related risk makes the insurance industry inevitably concerned with climate and climate change. Buildings hit by pluvial flooding is a key manifestation of this risk, giving rise to compensations of the induced physical damages and business interruptions. In this work, we establish a nationwide, building-specific risk score for water damage associated with pluvial flooding in Norway. We fit a generalized additive model that relates the number of water damages to a wide range of explanatory variables that can be categorized into building attributes, climatological variables and topographical characteristics. The model assigns a risk score to every location in Norway, based on local topography and climate, which is not only useful for insurance companies, but also for city planning. Combining our model with an ensemble of climate projections allows us to project the (spatially varying) impacts of climate change on the risk of pluvial flooding towards the middle and end of the 21st century.

==> latexmkrc <==
# HACK: this width seems to change with every compile, so
# latexmk runs latex too many times; ignore it
$hash_calc_ignore_pattern{'aux'} = 'statsocwidth';

# All the other default settings on Overleaf
# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}
